Data Security on Mobile Devices: Current State of the Art, Open Problems, and Proposed Solutions

In this work we present definitive evidence, analysis, and (where needed) speculation to answer the questions, (1) Which concrete security measures in mobile devices meaningfully prevent unauthorized access to user data? (2) In what ways are modern mobile devices accessed by unauthorized parties? (3) How can we improve modern mobile devices to prevent unauthorized access? We examine the two major platforms in the mobile space, iOS and Android, and for each we provide a thorough investigation of existing and historical security features, evidence-based discussion of known security bypass techniques, and concrete recommendations for remediation. We then aggregate and analyze public records, documentation, articles, and blog postings to categorize and discuss unauthorized bypass of security features by hackers and law enforcement alike. We provide in-depth analysis of the data potentially accessed via law enforcement methodologies from both mobile devices and associated cloud services. Our fact-gathering and analysis allow us to make a number of recommendations for improving data security on these devices. The mitigations we propose can be largely summarized as increasing coverage of sensitive data via strong encryption, but we detail various challenges and approaches towards this goal and others. It is our hope that this work stimulates mobile device development and research towards security and privacy, provides a unique reference of information, and acts as an evidence-based argument for the importance of reliable encryption to privacy, which we believe is both a human right and integral to a functioning democracy.

==> latexml_pre.tex <==
\renewcommand{\Gls}[1]{\MakeUppercase #1}
\renewcommand{\gls}[1]{#1}
\renewcommand{\makeglossaries}{}
\renewcommand{\newglossaryentry}[2]{}
\renewcommand{\printglossaries}{}
\renewenvironment{itemize*}{\begin{itemize}}{\end{itemize}}
\renewenvironment{tcolorbox}{\hline\\}{\hline\\}

\renewcommand*{\rot}[1]{\textbf{#1}}

\renewcommand{\bibliography}[1]{}
\renewcommand{\footnote}[1]{}
\renewcommand{\cite}[1]{}
\renewcommand{\footnotesize}{}
%\renewcommand{\url}[1]{$\texttt{#1}$}

\renewcommand{\mz}[1]{}
\renewcommand{\tj}[1]{}
\renewcommand{\mdg}[1]{}

